CFD analysis of electroviscous effects in electrolyte liquid flow through heterogeneously charged non-uniform microfluidic device

In this work, the pressure-driven flow of symmetric electrolyte liquid through a heterogeneously charged contraction-expansion (4:1:4) microfluidic device has been investigated numerically. Total potential ($U$), ion concentrations ($n_\pm$), velocity (${V}$), and pressure ($P$) fields are obtained after solving the mathematical model consisting of the Poisson's, Nernst-Planck (NP), Navier-Stokes (NS), and continuity equations numerically using the finite element method (FEM). Results are presented for wide ranges of dimensionless parameters such as inverse Debye length ($2\le K\le 20$), surface charge density ($4\le S_\text{1}\le 16$), and surface charge-heterogeneity ratio ($0\le S_\text{rh}\le 2$). Results show that the total potential ($\Delta U$) and pressure ($\Delta P$) drops change maximally by 3511.45% \add{(0.2127 to 7.6801)} (at $S_1=4$, $K=20$) and 41.4% \add{(1.0941 to 1.5471)} (at $S_1=16$, $K=2$), respectively with overall enhancing charge-heterogeneity ($0\le S_\text{rh}\le 2$), over the ranges of $K$ and $S_1$. Electroviscous correction factor, $Y$ (i.e., ratio of apparent to physical viscosity) increases maximally by 24.39\% \add{(1.1158 to 1.3879)} (at $K=4$, $S_\text{rh}=1.75$), 37.52% \add{(1.0597 to 1.4573)} (at $S_1=16$, $S_\text{rh}=2$), and 41.4% \add{(1.0306 to 1.4573)} (at $S_1=16$, $K=2$) with the variation of $S_1$ from 4 to 16, $K$ from 20 to 2, and $S_\text{rh}$ from 0 to 2, respectively. Further, overall increment in $Y$ is noted as 45.73\% \add{(1 to 1.4573)} (at $K=2$, $S_1=16$, $S_\text{rh}=2$), relative to non-EVF ($S_1=0$ or $K=\infty$). Thus, charge-heterogeneity enhances electroviscous effects in microfluidic devices, which enables the use of present numerical results for designing reliable and essential micro-sized channels for practical microfluidic applications.

==> Makefile <==
# type "make" command in Unix to create ps and pdf file 
#
#Colors
gray=\e[1;30m
red=\e[0;31m
RED=\e[1;31m
blue=\e[0;34m
BLUE=\e[1;34m
green=\e[0;32m
GREEN=\e[1;32m
cyan=\e[0;36m
CYAN=\e[1;36m
NC=\e[0m # No Color

# the documents to be compiled by default
# set defaultfile to the name of the main file without the .tex
#
defaultfile = $(foreach i,$(filter-out ,$(shell grep -l documentclass *.tex)), $(basename $i))
#
ASPELL = aspell -t -c --mode=tex
ISPELL = ispell -t  --mode=tex
LATEX = latex -interaction=batchmode
BIBTEX = bibtex 
MAKEINDEX = makeindex
PDFLATEX = pdflatex -interaction=batchmode
#
DVIPS = dvips -Pwww
DVIPDF = dvipdf 
PSPDF = ps2pdf
#
all: pdf clean
#
pdf:
	@echo -e ""
	@echo -e "$(BLUE)====> Default file being compiled: $(RED)$(defaultfile).tex$(NC)"
	@echo -e ""
	@echo -e "$(BLUE)====> $(green)Running LaTeX$(NC)" ;
	$(LATEX) $< $(QUIET)$(defaultfile)
#
#	@echo -e "$(BLUE)====> $(green)Running PDFLaTeX to generate PDF document$(NC)" ;
#	$(PDFLATEX) $< $(QUIET)$(defaultfile)
#
	@echo -e "$(BLUE)====> $(green)Running BibTex$(NC)" ;
	$(BIBTEX) $< $(QUIET)$(defaultfile)
#	
#	@echo -e "$(BLUE)====> $(green)Running aspell$(NC)" ;
#	$(ASPELL) $< $(QUIET)$(defaultfile).tex
#
#	@echo -e "$(BLUE)====> $(green)Running ispell$(NC)" ;
#	$(ISPELL) $< $(QUIET)$(defaultfile).tex
#
	@echo -e "$(BLUE)====> $(green)Running Makeindex$(NC)" ;
	$(MAKEINDEX) $< $(QUIET)$(defaultfile).nlo -s nomencl.ist -o  $(QUIET)$(defaultfile).nls
#
#	@echo -e "$(BLUE)====> $(green)Running PDFLaTeX to generate PDF document$(NC)" ;
#	$(PDFLATEX) $< $(QUIET)$(defaultfile)
#
#	@echo -e "$(BLUE)====> $(green)Running PDFLaTeX to generate PDF document$(NC)" ;
#	$(PDFLATEX) $< $(QUIET)$(defaultfile)
#
#
	@echo -e "$(BLUE)====> $(green)Running LaTeX$(NC)" ;
	$(LATEX) $< $(QUIET)$(defaultfile)
#
	@echo -e "$(BLUE)====> $(green)Running LaTeX$(NC)" ;
	$(LATEX) $< $(QUIET)$(defaultfile)
#
	@echo -e "$(BLUE)====> $(green)Generating PS document from DVI document$(NC)" ;
	$(DVIPS) $< $(QUIET)$(defaultfile)
#
	@echo -e "$(BLUE)====> $(green)Generating PDF document from DVI document$(NC)" ;
	$(DVIPDF) $< $(QUIET)$(defaultfile)
#
#	@echo -e "$(BLUE)====> $(green)Generating PDF document from PS document$(NC)" ;
#	$(PSPDF) $(defaultfile).ps $(defaultfile).pdf
#
clean:
	@echo -e "$(RED)====> $(red)Cleaning up temporary files$(NC)"
	rm -f *.brf *.glo *.ist *.nlo  *.out *.spl *.log *.aux *.*% *.lof *.gls *.nls
	rm -f *.lop *.lot *.toc *.idx *.ilg *.ind *.bbl *.blg *.backup *.bak *~



